An Improved Fully Dynamic Algorithm for Counting 4-Cycles in General Graphs using Fast Matrix Multiplication

We study subgraph counting over fully dynamic graphs, which undergo edge insertions and deletions. Counting subgraphs is a fundamental problem in graph theory with numerous applications across various fields, including database theory, social network analysis, and computational biology. Maintaining the number of triangles in fully dynamic graphs is very well studied and has an upper bound of O(m^{1/2}) for the update time by Kara, Ngo, Nikolic, Olteanu, and Zhang (TODS 20). There is also a conditional lower bound of approximately Omega(m^{1/2}) for the update time by Henzinger, Krinninger, Nanongkai, and Saranurak (STOC 15) under the OMv conjecture implying that O(m^{1/2}) is the ``right answer'' for the update time of counting triangles. More recently, Hanauer, Henzinger, and Hua (SAND 22) studied the problem of maintaining the number of 4-cycles in fully dynamic graphs and designed an algorithm with O(m^{2/3}) update time which is a natural generalization of the approach for counting triangles. Thus, it seems natural that O(m^{2/3}) might be the correct answer for the complexity of the update time for counting 4-cycles. In this work, we present an improved algorithm for maintaining the number of 4-cycles in fully dynamic graphs. Our algorithm achieves a worst-case update time of O(m^{2/3-eps}) for some constant eps>0. Our approach crucially uses fast matrix multiplication and leverages recent developments therein to get an improved runtime. Using the current best value of the matrix multiplication exponent omega=2.371339 we get eps=0.009811 and if we assume the best possible exponent i.e. omega=2 then we get eps=1/24. The lower bound for the update time is Omega(m^{1/2}), so there is still a big gap between the best-known upper and lower bounds. The key message of our paper is demonstrating that O(m^{2/3}) is not the correct answer for the complexity of the update time.

==> OpenProblems.tex <==
% !TeX root = main.tex 
%!TEX root = main.tex

\section{Open Problems}\label{sec:open-probs}




==> alg.tex <==
%% !TeX root = main.tex 
%%!TEX root = main.tex
%
%\section{The Fast Algorithm using FMM}\label{sec:Algorithm}
%
%
%\subsection{Setup}
%
%We have four layers $L_1,L_2,L_3$ and $L_4$ each containing $n$ vertices.
%Let the edges between the four consecutive layers be represented by the matrices $A, B, C, D$. 
%We assume without loss of generality that we have to answer queries only when there is an edge 
%update in $D$ where the query is the new number of cycles i.e. the number of cycles going 
%through 
%the query edge.
%We maintain a data structure that helps us answer queries in $D$, and we maintain the same data 
%structure for all matrices $A,B,C$ and $D$. The analysis is the same for all of them, so we just 
%focus 
%on queries in $D$ and edge updates everywhere else.
%Note that answering a query that outputs the total number of cycles is equivalent to answering the 
%number of new cycles i.e. the ones passing through the last edge.
%Here we have reduced the problem to answering queries $(u,v)$ only when they are in layer $D$ 
%which is equivalent to outputting the number of paths between $u$ and $v$.
%
%%We consider graphs where the number of edges $m = O(n^{1.5})$.
%%This is a big assumption that we need to try and eventually get rid of.
%%Another assumption is that there are only edge insertions but this should not be too hard to 
%%remove.
%We let the worst-case update time be $O(m^{2/3-\eps})$ and we will show we can get $\eps>0$.
%We first discuss the data structures we need to store and then show how the queries can be 
%answered in time $O(m^{2/3-\eps})$.
%Before we discuss the data structures we need, we partition the vertices into different classes.
%We first discuss \emph{tiny} ($T$) vertices.
%%All the vertices in the graph are either easy or non-easy and the non-easy vertices are 
%%partitioned 
%%into other classes which we discuss later.
%The vertices in $L_1$ (resp. $L_4$) are in $T$ when their degree in $A$ (resp. $C$) is at most 
%$m^{1/3-2\eps}$.
%The vertices in $L_2$ (resp. $L_3$) are in $T$ when their combined degree in $A,B$ (resp. 
%$B,C$) 
%is at most $m^{1/3-2\eps}$.
%%The setup that follows is \emph{only} for \emph{non-easy} vertices.
%
%The vertices in $L_1$ and $L_4$ are partitioned into $H,M,L$ (other than $T$) based on their 
%degree in $A$ and $C$ respectively.
%Vertices with degree in $A$ (resp. $C$) at most $m^{1/3+\eps}$ are in $L$ (\emph{low}), at least 
%$m^{2/3-\eps}$ are in $H$ (\emph{high}) and the remaining ones are in $M$ (\emph{medium}).
%
%We partition vertices in $L_2$ (resp. $L_3$) into \emph{dense} ($D$) and \emph{sparse} ($S$) 
%based on their combined degree in $A,B$ (resp. $B,C$).
%Vertices in $L_2$ (resp. $L_3$) with degree in $A,B$ (resp. $B,C$) at most $m^{2/3-\eps}$ are in 
%$S$ and the others are in $D$.
%%We also partition vertices in $L_2$ (resp. $L_3$) into \emph{fat} ($F$) and 
%%\emph{thin} ($T$) based on their combined degree in $A$ and $B$ (resp. $B$ and $C$).
%%Vertices with degree in $A,B$ (resp. $B,C$) at most $m^{2/3-\eps}$ are in $T$ and the others 
%%are 
%%in 
%%$F$.
%
%We use superscripts to talk about a submatrix of a matrix by restricting the vertices in different 
%layers. For instance $A^{H D}$ represents the submatrix of $A$ where we only look at the edges 
%of 
%$A$ between $L_1^H$ and $L_2^D$. We also use $A$ to represent all 
%the vertices in a layer.
%We use a subscript to represent a subset of the edges.
%To make things less cumbersome we will drop some parts of the notation when things are clear 
%from 
%context.
%
%\vihan{say we will ignore leading constants in analysis? No, mention constant exactly}
%
%
%
%\subsection{Tiny vertices}
%
%In this subsection, we describe how we handle paths that go through tiny vertices and answer 
%queries when at least one endpoint is a tiny vertex.
%For the remainder of the analysis we can completely ignore tiny vertices.
%
%\paragraph{Data Structure for Tiny vertices}
%We show the data structures we need to store to calculate the number of paths through tiny 
%vertices 
%and to answer queries with tiny vertices in them.
%
%We maintain the data structures: $A^{AT} B^{TA},$ $B^{AT}C^{TA},$ $A^{AS}B^{SA},$ 
%$B^{AS}C^{SA}$.
%
%\begin{claim}\label{clm:T-DS}
%	The worst-case update time for these data structures for tiny and sparse vertices is 
%	$O(m^{2/3-\eps})$.
%\end{claim}
%\begin{proof}
%	Consider the data structure $A^{AS} B^{SA}$. The analysis for the others is identical.
%	If there is an update $(u,v)$ in $A^{AS}$ then we go over the $m^{2/3-\eps}$ neighbors of $v$ 
%	in $L_3$ and update the number of paths in the data structure. 
%	If the update $(u,v)$ is in $B^{SA}$ then we iterate 
%	over the $m^{2/3-\eps}$ neighbors of $u$ in $L_1$ and update the number of paths.
%\end{proof}
%
%We maintain some data structures just for high and medium degree vertices: 
%$A^{HT}B^{TT}C^{TH},$ 
%$A^{MT}B^{TT}C^{TH},$ $A^{HT}B^{TT}C^{TM}$.
%
%\begin{claim}\label{clm:HM-T-DS}
%	The worst-case update time for these data structures for high and medium degree vertices is 
%	$O(m^{2/3-\eps})$.
%\end{claim}
%\begin{proof}
%	Consider the data structure $A^{HT}B^{TT}C^{TM}$. The analysis for the others is 
%	identical.
%	First we note that we already have the data structures $A^{AT} B^{TA}, B^{AT}C^{TA}$ stored.
%	This gives us access to $A^{HT} B^{TT}$ and $B^{TT}C^{TM}$.
%	
%	If there is an update $(u,v)$ in $A^{HT}$ then we go over the $m^{2/3-\eps}$ vertices in 
%	$L_4^M$ and update the number of paths using $B^{TT}C^{TM}$.
%	Similarly, if there is an update $(u,v)$ in $C^{TM}$ then we go over the $m^{1/3+\eps}$ vertices 
%	in $L_1^H$ and update the number of paths using $A^{HT} B^{TT}$.
%	
%	Finally, if there is an update $(u,v)$ in $B^{TT}$ then we go over the $m^{1/3-2\eps}$ neighbors 
%	of $u,v$ in $L_1^H$ and $L_4^M$ and update the number of paths in the data structure. 
%	The total number of pairs is $m^{2/3-4\eps}$, so we are done.
%\end{proof}
%
%
%We maintain additional data structures for high degree vertices: $A^{HT}B^{TS}C^{SH}, 
%A^{HS}B^{ST}C^{TH}$.
%
%\begin{claim}\label{clm:HT-DS}
%	The worst-case update time for these data structures for high degree vertices is 
%	$O(m^{2/3-\eps})$.
%\end{claim}
%\begin{proof}
%	Consider the data structure $A^{HT}B^{TS}C^{SH}$. The analysis for $A^{HS}B^{ST}C^{TH}$ is 
%	identical.
%	First we note that we already have data structures $A^{AT} B^{TA}$ and $B^{AS}C^{SA}$ 
%stored.
%	This gives us access to $A^{HT} B^{TS}$ and $B^{TS}C^{SH}$.
%	
%	If there is an update $(u,v)$ in $A^{HT}$ then we go over the $m^{1/3+\eps}$ vertices in 
%	$L_4^H$ and update the number of paths using $B^{TS}C^{SH}$.
%	Similarly, if there is an update $(u,v)$ in $C^{SH}$ then we go over the $m^{1/3+\eps}$ vertices 
%	in $L_1^H$ and update the number of paths using $A^{HT} B^{TS}$.
%	
%	Finally, if there is an update $(u,v)$ in $B^{TS}$ then we go over the $m^{1/3-2\eps}$ neighbors 
%	of $u$ in $L_1^H$ and also the $m^{1/3+\eps}$ vertices in $L_4^H$ and update the number of 
%	paths in the data structure. 
%	The total number of pairs is $m^{2/3-\eps}$, so we are done.
%\end{proof}
%
%\paragraph{Queries for tiny vertices}
%Here we show how to answer queries when at least one of the vertices in the query is a tiny vertex.
%
%\textbf{Case 1: TT, TL} \\
%If one vertex is in $T$ and the other in $T,L$ then we can still iterate over both of their neighbors 
%in 
%time $m^{2/3-\eps}$ and then look at the number of paths.
%
%\textbf{Case 2: TM, TH} \\
%If one vertex is in $T$ and the other in $H,M$ then we can first calculate the number of paths that 
%go 
%through $L_3^D$.
%This is done by iterating over the $m^{1/3-2\eps}$ neighbors of $u$ and all $m^{1/3+\eps}$ 
%vertices 
%in $L_3^D$ and checking if they form a path.
%The time taken is $m^{2/3-\eps}$.
%
%We can iterate over the $m^{1/3-2\eps}$ neighbors of $u$ and then use the data structure 
%$B^{AS}C^{SA}$ to get the number of paths going through $L_3^S$ and use $B^{AT}C^{TA}$ to 
%get the number of paths going through $L_3^T$.
%
%\paragraph{Paths through tiny vertices}
%Now we need to show that we can easily calculate the number of paths through tiny vertices in 
%$L_2$ and $L_3$ no matter what kind of query we get.
%Once we do this we can ignore tiny vertices for the rest of the analysis.
%
%We first describe queries where there are no high degree vertices.
%\begin{claim}
%	We can calculate the number of paths through tiny vertices in $L_2$ or $L_3$ in time 
%	$m^{2/3-\eps}$ when the query does not contain a high degree vertex. 	
%\end{claim}
%\begin{proof}
%	Let the query be $u,v$. 
%	We have the data structures $A^{AT} B^{TA}$ and $B^{AT} C^{TA}$ stored.
%	We iterate over neighbors of $u$ in $m^{2/3-\eps}$ time and use $B^{AT} C^{TA}$ to get the 
%paths 
%	that go to $v$ via $L_3^T$.
%	We can do the same side from the side of $v$ and get the paths through $L_2^T$.
%	Note that we will calculate the $TT$ paths just once.
%\end{proof}
%
%We can now see why the above procedure does not work for high degree vertices.
%High degree vertices have too many neighbors to iterate over.
%So we handle these cases separately.
%
%\textbf{Case 1: HH} \\
%We can easily get the number of $TT$ paths using $A^{HT}B^{TT}C^{TH}$ and $TS$ paths using 
%$A^{HT}B^{TS}C^{SH}$. 
%Finally, for the number of $TD$ paths, we iterate over the $m^{1/3+\eps}$ neighbors of $v$ in 
%$L_3^D$ and then use the data structure $A^{AT}B^{TA}$ to get the number of paths to $u$ via 
%$L_2^T$.
%The other paths can be found symmetrically.
%
%\textbf{Case 2: HM} \\
%We can easily get the number of $TT$ paths using $A^{HT}B^{TT}C^{TM}$.
%For the number of $TD$ paths (and $DT$ paths) we iterate over the $m^{1/3+\eps}$ neighbors of 
%$v$ 
%in $L_3^D$ and then use the data structure $A^{AT}B^{TA}$ to get the number of paths to $u$ 
%via 
%$L_2^T$.
%To get the number of $ST$ and $TS$ paths we iterate over the $m^{2/3-\eps}$ neighbors of $v$ 
%and 
%then use $A^{AS}B^{SA}$ to get the number of $ST$ paths and use $A^{AT}B^{TA}$ to get the 
%number of $TS$ paths.
%
%\textbf{Case 3: HL} \\
%To find the number of $AT$ paths we can iterate over the neighbors of neighbors of $v$ and 
%check if 
%they have an edge to $u$. This takes $m^{1/3+\eps} \cdot m^{1/3-2\eps}=m^{2/3-\eps}$ time.
%For the number of $TA$ paths we can iterate over the neighbors of $v$ and use $A^{AT}B^{TA}$.
%
%
%This means that we can figure out the number of paths through tiny vertices, and we can also 
%answer 
%queries when they involve tiny vertices, so we can completely ignore tiny vertices in the rest of the 
%analysis.
%This means that we can assume that each layer has at most $m^{2/3+2\eps}$ vertices because all 
%the 
%remaining vertices have degree at least $m^{1/3-2\eps}$.
%
%\vihan{Later when we use A do we mean with or without tiny vertices? This will be imp for class 
%transition. maybe have $\bar{T}$ for $A-T$}
%
%\subsection{Phases}
%
%We define a \emph{phase} as $m^{\delta}$ edge insertions. 
%A phase should be long enough to multiply two square matrices of dimension $m^{2/3+2\eps}$.
%The amount of time it takes using fast matrix multiplication is $m^{\omega \cdot (2/3 +2\eps)}$.
%Thus, we have $m^{\delta} \cdot m^{2/3-\eps} \geq m^{\omega \cdot (2/3+2\eps)}$, and so we 
%set: 
%\[\delta: = 
%0.916 + 3.4\eps. \tag{since $0.916 > 1.372 \times 0.667$}
%\]
%Thus, the number of vertices with degree at least $m^{2/3-\eps}$ is at most 
%$m^{\delta-2/3+\eps}\leq 
%m^{0.256+4.4\eps}$.
%We call such vertices in $L_2$ and $L_3$ \emph{dense in a phase} and call the others 
%\emph{sparse in a phase}.
%
%Note that during a phase we can compute all matrix products of the previous phase (for $A,B,C,D$ 
%in that phase).
%So we can divide all the phases into two parts $\pnew$ which contains the current phase 
%$P_{j+1}$ and the phase just before it $P_{j}$. All phases older than that are represented by 
%$\po$. 
%The edges in $A$ that are part of $\po$ are represented by $\ao$ and those that are part of 
%$\pnew$ are represented by $\anew$ (similar for $B,C$).
%
%So the new phase has at most $2 m^{\delta}$ edges but the old phase can have $O(m)$ 
%edges.
%For the new phase to have asymptotically fewer edges we need $\delta<1$ and this happens only 
%when $\omega < 2.5 -O(\eps)$ which in particular happens only when $\omega<2.5$.
%This is very surprising because any value of $\omega$ better than $3$ is not sufficient.
%
%\subsection{Data Structures for vertices in $H,M$}
%
%In this subsection, we discuss the data structures we store for the high and medium degree 
%vertices 
%in $L_1$ and $L_4$.
%We maintain the following data structures: $A^{HD} B^{DD}, B^{DD} C^{DH}$ and $A^{MD} 
%B^{DD}, 
%B^{DD} C^{DM}$.
%
%Notice that we can always update these data structures for any edge update in $m^{2/3-\eps}$ 
%time. 
%The reason for this is that the maximum size of these restricted layers is at most $m^{2/3-\eps}$.
%\begin{claim}\label{clm:HM-DS}
%	The worst-case update time for these data structures for high and medium degree vertices is 
%	$O(m^{2/3-\eps})$.
%\end{claim}
%\begin{proof}
%%	Consider the data structure $A^{MS} B^{SA}$.
%%	If there is an update $(u,v)$ in $A^{MS}$ then we go over the $m^{2/3-\eps}$ neighbors of 
%%$v$ 
%%	and update the number of paths in the data structure. If the update is in $B^{SA}$ then we 
%%iterate 
%%	over the $m^{2/3-\eps}$ vertices in $L_1^M$ and update the number of paths.
%%	The analysis is similar for $B^{AS} C^{SM}$.
%	Consider the data structure $A^{MD} B^{DD}$.
%	If there is an update $(u,v)$ in $A^{MD}$ then we go over the $m^{1/3+\eps}$ neighbors of $v$ 
%in 
%	$L_3^D$ and update the number of paths in the data structure. If the update is in $B^{DD}$ 
%then 
%	we iterate over the $m^{2/3-\eps}$ vertices in $L_1^M$ and update the number of paths.
%	The analysis is similar for $ B^{DD} C^{DM}$.
%	
%	The same arguments work for high degree vertices. This concludes the proof.
%\end{proof}
%
%
%We maintain additional data structures for high degree vertices: $\anew^{HS} \bnew^{SS} 
%\cnew^{SH},$ $\anew^{HS} \bnew^{SS} \co^{SH}, \ldots$. This list includes all possible 
%combinations of old and new phases other than $\ao^{HS} \bnew^{SS} \co^{SH}$ and $\ao^{HS} 
%\bo^{SS} \co^{SH}$.
%
%\begin{claim}\label{clm:H-DS}
%	The worst-case update time for the additional data structures for high degree vertices is 
%	$m^{2/3-\eps}$.
%\end{claim}
%\begin{proof}
%	We know that we can store the data structures of the form $A^{HS} B^{SA}$ and $B^{AS} 
%	C^{SH}$ (\vihan{cite}) for all combinations of old and new phases.
%	
%	Say we get an edge update in $A$ (resp. $C$) then we can go over all vertices $m^{1/3+\eps}$ 
%in 
%	$L_4^H$ (resp. $L_1^H$) and update the number of paths. 
%	This is possible since we have the number of $B^{AS} C^{SH}$ (resp. $A^{HS} B^{SA}$) paths 
%	stored.
%	
%	If we get an edge update in $B$ then we iterate over all pairs of vertices in $L_1^H$ and 
%$L_4^H$ 
%	and update the data structure.
%	This seems like it will take too much time on the surface, but we know that the data structure has 
%	either $A$ or $C$ in the new phase and hence the number of high degree vertices in a new 
%phase is 
%	at most $m^{\delta -2/3 +\eps}$ as opposed to $m^{1-2/3+\eps}$.
%	
%	Thus, iterating over all pairs of high vertices takes time $m^{1/3+\eps} \cdot m^{\delta - 
%2/3+\eps} 
%	\leq m^{2/3-\eps}$.
%\end{proof}
%
%This gives us a constraint: $\delta \leq 1-3\eps$ which gives us the following bound on $\eps$:
%	\begin{tcolorbox}
%	\begin{equation}\label{eq:HH-pairs-new_old}		
%		\eps \leq 0.013125
%	\end{equation}
%\end{tcolorbox}
%
%
%\subsection{Data structures for vertices in $L$}
%
%In this subsection, we mention the data structures we need for low degree vertices: $\anew^{AD} 
%\bo^{DD},$ $\bo^{DD} \cnew^{DA}$.
%Note that this data structure is for all vertices, but we use it only for low degree vertices.
%
%\begin{claim}\label{clm:L-DS}
%	The worst-case update time for the data structures for low degree vertices is 
%	$m^{1/3+\eps}$.
%\end{claim}
%\begin{proof}
%	Observe that we only deal with $\bo$ and not $\bnew$ so there are no updates in $B$.
%	If there are any updates in $A$ or $C$ then we iterate over all its dense neighbors in 
%	$m^{1/3+\eps}$ time and update the data structure.
%\end{proof}
%
%\subsection{Queries with vertices in only $H,M$:}
%
%There are two choices for vertices in $L_2$ and $L_3$, sparse or dense, so there are four kinds of 
%paths between any pair of vertices in $L_1$ and $L_4$.
%Consider paths where there is at least one dense vertex. 
%We can iterate over the all the $m^{1/3+\eps}$ dense vertices in that layer and check for an edge 
%to 
%one side and then the number of paths to the other side.
%This can be done using the data structures of the form $A^{HD}B^{DD}$ for paths through dense 
%vertices and $A^{AS}B^{SA}$ for paths through sparse vertices.
%
%So now we only worry about paths that go through $L_2^S$ and $L_3^S$.
%If one of the vertices in the query is in $M$ then we iterate over its $m^{2/3-\eps}$ sparse 
%neighbors 
%and use the number of sparse paths to the other endpoint of the query stored in the data 
%structure of the form $A^{AS}B^{SA}$.
%
%The remaining case is where the query has both high degree endpoints, and we need to calculate 
%the 
%number of $SS$ paths.
%We know the number of $\ao \bo \co$ paths from the matrix product of the previous phase.
%We also know the number of $\ao \bnew \co$ paths from the simple algorithm where $A,C$ are 
%fixed.
%For the remaining combination of phases we have data structures where the number of paths are 
%explicitly stored.
%
%
%
%\subsection{Queries with at least one vertex in $L$}
%
%Let the current query be $e=(u,v)$ where $u$ is in $L_1$ and $v$ is in $L_4$.
%
%\paragraph{HL, ML queries:}
%In this case, $u \in L_1^H$ is a high degree vertex and $v \in L_4^L$ is a low degree vertex.
%
%We can iterate over all $m^{1/3 +\eps}$ neighbors $w_i$ of $v$. We know the number of $DD, SS, 
%SD$ paths from $u$ to $w_i$'s using the data structures $A^{AS} B^{SA}$ and $A^{HD} 
%B^{DD}$. 
%For the $DS$ paths we iterate over the $m^{1/3+\eps}$ neighbors of $u$ in $L_2^D$ and use 
%$B^{AS}C^{SA}$ to get the number of paths to $v$ via $L_3^S$.
%
%Note that the proof is identical for $ML$ queries.
%
%\paragraph{LL queries:}
%In this case, $u \in L_1^L$ and $v\in L_4^L$ are both low degree vertices.
%
%It is easy to find the number of $SS,SD,DS$ paths by going over the neighbors of a query vertex 
%and 
%then using the data structures $A^{AS}B^{SA}, B^{AS}C^{SA}$.
%So we now only worry about $DD$ paths.
%
%\textbf{Case 1:} $\ao \bo \co, \ao \bo \cnew, \anew \bo \co$ \\
%Consider $\ao \bo \cnew$ paths (the others are symmetric).
%We can iterate over the $m^{1/3+\eps}$ neighbors of $v$ and use the number of $\ao \bo$ paths 
%stored in the matrix product.
%
%\textbf{Case 2:} $\anew \bo \cnew$ \\
%We have the following data structures stored: $\anew^{LD} \bo^{DD}, \bo^{DD} \cnew^{DL}$.
%Iterate over the $m^{1/3+\eps}$ neighbors of $u$ and use the number of $DD$ paths to $v$.
%
%\textbf{Case 3:} $\ao \bnew \co,$ $\anew \bnew \cnew,$ $\anew \bnew \co,$ $\ao \bnew \cnew$ \\
%We go over all pairs of dense vertices in $L_2,L_3$ in time $m^{2(\delta +\eps -2/3)} \leq 
%m^{2/3-\eps}$ and check if they form a path.
% 
%
%\subsection{Vertices changing classes}
%Note that till now we have assumed that the classes of vertices are fixed. But if the degree of 
%vertices change then their classes will change too. So in this subsection, we describe what 
%happens 
%when the degree of the vertices changes by a lot, and it has to change classes.
%
%We slightly adjust the thresholds between classes.
%Say the threshold between two classes is $x$.
%When the degree of the vertex is between $x$ and $2x$ we will say that the vertex still belongs to 
%the old class and is transitioning to the new class.
%Observe that this might change the previous bounds but only by constant factors.
%
%During this period we will develop data structures of both classes for this vertex.
%Note that this computation will only be done when we get an edge incident to this vertex so by the 
%time its degree doubles we have the new data structure ready.
%This ensures that during an edge update we are doing this computation for at most $2$ vertices 
%and 
%thus does not mess up the worst-case update time.
%Finally, when the vertex enters the transition range, we partition the edges into the ones that came 
%before and after that moment and deal with them separately.
%The main task is to compute the data structure for the edges that come before the transition 
%moment in time $O(x \cdot m^{2/3-\eps})$.
%
%
%\textbf{Case 1: $L$ and $M$} \\
%Notice that the data structures for $L$ are a subset of those of $M$.
%So we will focus on vertices transitioning from $L$ to $M$.
%The amount of time we have is $m^{1/3+\eps} \cdot O(m^{2/3-\eps}) = O(m)$.
%
%\begin{claim}
%	The amount of time it takes to update the data structures $A^{MD} B^{DD}, B^{DD} C^{DM}$ for 
%	a vertex $v$ transitioning from $L$ to $M$ is $O(m)$.
%\end{claim}
%\begin{proof}
%	Consider the data structure $A^{MD} B^{DD}$ (the proof for the other one is similar).
%	We can iterate over all neighbors of $v$ in $L_2^D$ and then go over all their neighbors in 
%	$L_3^D$ to update the number of paths.
%	This takes time $m^{1/3+\eps} \cdot m^{1/3+\eps}$ that is within our budget.
%	
%	If there is any new edge update in $\bnew$ then we can go over all transitioning vertices in 
%$L,M$ 
%	and update the data structure in time $m^{1/3+\eps}$ which is within the budget for update time. 
%\end{proof}
%
%\begin{claim}
%	The amount of time it takes to update the data structures $A^{MT} B^{TT} C^{TH} ,$ $A^{HT} 
%	B^{TT} C^{TM}$ for a vertex $v$ transitioning from $L$ to $M$ is $O(m)$.
%\end{claim}
%\begin{proof}
%	Consider the data structure $A^{MT} B^{TT} C^{TH}$ for a vertex $v\in L_1$.
%	We can iterate over all neighbors of $v$ in $L_2^T$ and then go over all their neighbors in 
%	$L_3^T$ and finally over their neighbors in $L_4^H$ to update the number of paths.
%	This takes time $m^{1/3+\eps} \cdot m^{2/3-4\eps}=m^{1-3\eps}$ that is within our budget.
%\end{proof}
%
%\textbf{Case 2: $M$ and $H$} \\
%Notice that the data structures for $M$ are a subset of those for $H$.
%So we will focus on a vertex $v\in L_1$ transitioning from $M$ to $H$.
%The amount of time we have is at least $m^{2/3-\eps} \cdot O(m^{2/3-\eps})$.
%
%The first type of extra data structures are of the form $A^{HT} B^{TS} C^{SH},$ $A^{HS} B^{ST} 
%C^{TH}$.
%\begin{claim}
%	The amount of time it takes to update the data structures $A^{HT} B^{TS} C^{SH},$ $A^{HS} 
%	B^{ST} C^{TH}$ for a vertex 
%	$v\in L_1$ transitioning from $M$ to $H$ is $O(m^{4/3-2\eps})$.
%\end{claim}
%\begin{proof}
%	Consider the data structure $A^{HT} B^{TS} C^{SH}$.
%	We can go over all $m^{2/3-\eps}$ neighbors of $v$ in $L_2^T$ and all their $m^{1/3-2\eps}$ 
%	neighbors in $L_3^S$ and finally all $m^{1/3+\eps}$ vertices in $L_4^H$ and update the 
%number of 
%	paths.
%	The time taken is $m^{2/3-\eps} \cdot m^{1/3-2\eps} \cdot m^{1/3+\eps} = m^{4/3-2\eps}$.
%	
%	Consider the data structure $A^{HS} B^{ST} C^{TH}$.
%	We can go over all $m^{2/3-\eps}$ neighbors $w_i$ of $v$ in $L_2^S$, but we cannot iterate 
%over 
%	their neighbors.
%	So we also iterate over all $m^{1/3+\eps}$ vertices $u_i$ in $L_4^H$ and then us the data 
%structure 
%	$B^{AT}C^{TA}$ to get the number of paths between $w_i$ and $u_j$ through $L_3^T$. 
%	This takes time $m^{2/3-\eps} \cdot m^{1/3+\eps} \leq m^{4/3-2\eps}$.
%\end{proof}
%
%
%Note that we have data structures that calculate the number of paths through vertices in 
%$L_2,L_3$, 
%so we need to be careful not to over count the number of paths.
%When the vertex enters the transition phase we keep it in the old class for answering queries, while 
%constructing its data structure for the new class.
%Counter-intuitively, we also need to create its data structure for the old class.
%For both classes, we create a new data structure for the transitioning vertices and maintain it 
%separately.
%
%Once the vertex exits the transition range and crosses over into one of the classes, we update the 
%main data structure. 
%If it transitions into the old class then we do not have to do anything to the old data structure, and 
%we 
%can delete the new data structure we computed for it.
%If it transitions into the new class then we update the main data structure with the new data 
%structure 
%we maintained separately.
%We also update the data structure for the old class, using the new data structure we maintained 
%separately, by subtracting its contribution (this is why we needed to create its data structure for 
%the 
%old class).
%
%\textbf{Case 3: $S$ and $D$} \\
%Consider vertices transitioning from $S$ to $D$.
%The amount of time we have is $m^{2/3-\eps} \cdot O(m^{2/3-\eps})$.
%The data structures we need to create are of the form $A^{HD} B^{DD},$ $A^{MD} B^{DD},$ 
%$\anew^{AD} \bo^{DD}$.
%
%\begin{claim}
%	The amount of time it takes to create the data structure $A^{MD} B^{DD}$ for a vertex 
%	$v$ transitioning from $S$ to $D$ is $O(m^{4/3-2\eps})$.
%\end{claim}
%\begin{proof}
%	We go over all $m^{2/3-\eps}$ neighbors in $L_1$ and all $m^{1/3+\eps}$ 
%	dense vertices and create the data structure in time $m \leq m^{4/3-2\eps}$.
%\end{proof}
%
%Consider vertices transitioning from $D$ to $S$.
%The amount of time we have is at least $m^{2/3-\eps} \cdot O(m^{2/3-\eps})$.
%Consider the data structures of the form $A^{AS} B^{SA}$.
%
%\begin{claim}
%	The amount of time it takes to create the data structure $A^{AS} B^{SA}$ for a vertex 
%	$v$ transitioning from $D$ to $S$ is $O(m^{4/3-2\eps})$.
%\end{claim}
%\begin{proof}
%	We go over all pairs of $m^{2/3-\eps}$ neighbors on both sides and create the data structure.
%\end{proof}
%
%
%We now, consider the data structures of the form $\ao^{HS} \bo^{SS} \cnew^{SH}$.
%\begin{claim}
%	The amount of time it takes to create the data structures of the form $A^{HS} B^{SS} C^{SH}$  
%	for a vertex $v$ transitioning from $D$ to $S$ is $O(m^{4/3-2\eps})$.
%\end{claim}
%\begin{proof}
%	We go over all $m^{2/3-\eps}$ neighbors of $v$ in $L_3^S$ and also all pairs of high degree 
%	vertices in $L_1$ and $L_4$ and create the data structure.
%	On the surface this seems like it takes too much time but note that all the relevant data 
%structures 
%	of this type have either $A$ or $C$ in the new phase, and so we can iterate over all pairs of high 
%	degree vertices in 
%	time $m^{2/3-\eps}$.
%	This gives us the desired bound of $O(m^{4/3-2\eps})$ for the update time.
%\end{proof}
%
%Finally, consider the data structures of the form $A^{HS} B^{ST} C^{TH}$.
%\begin{claim}
%	The amount of time it takes to create the data structures of the form $A^{HS} B^{ST} C^{TH}$  
%	for a vertex $v\in L_2$ transitioning from $D$ to $S$ is $O(m^{2/3+2\eps})$.
%\end{claim}
%\begin{proof}
%	We go over all $m^{1/3+\eps}$ neighbors of $v$ in $L_1^H$ and also all $m^{1/3+\eps}$ high 
%	degree vertices $w_i$ in $L_4$. 
%	We then use the number of paths between $v$ and $w_i$ through $L_3^T$ stored in 
%	$B^{AT}C^{TA}$ and create the data structure.	
%	This gives us the desired bound of $O(m^{2/3+2\eps})$ for the update time.
%\end{proof}
%
%
%\textbf{Case 4: $T$ and $S$} \\
%Note that both $T,L$ do not have any data structures in $L_1,L_4$, so we do not have a transition 
%between $T$ and $L$.
%We now consider the transition between $T$ and $S$.
%First consider vertices transitioning from $T$ to $S$.
%The amount of time we have is $m^{1/3-2\eps} \cdot m^{2/3-\eps}=m^{1-3\eps}$.
%
%\begin{claim}
%	The amount of time it takes to create the data structure $A^{AS} B^{SA}$ for a vertex 
%	$v$ transitioning from $T$ to $S$ is $O(m^{2/3-4\eps})$.
%\end{claim}
%\begin{proof}
%	We go over all pairs of $m^{1/3-2\eps}$ neighbors on both sides and create the data structure.
%\end{proof}
%
%We now, consider the data structures of the form $\ao^{HS} \bo^{SS} \cnew^{SH}$.
%\begin{claim}
%	The amount of time it takes to create the data structures of the form $A^{HS} B^{SS} C^{SH}$  
%	for a vertex $v \in L_2$ transitioning from $T$ to $S$ is $m^{1-3\eps}$.
%\end{claim}
%\begin{proof}
%	We go over all $m^{1/3-2\eps}$ neighbors of $v$ in $L_3^S$ and also all pairs of high degree 
%	vertices in $L_1$ and $L_4$ and create the data structure.
%	On the surface this seems like it takes too much time but note that all the relevant data 
%structures 
%	of this type have either $A$ or $C$ in the new phase, and so we can iterate over all pairs of high 
%	degree vertices in time $m^{2/3-\eps}$.
%	This gives us the desired bound of $m^{1-3\eps}$ for the update time.
%\end{proof}
%
%Finally, consider the data structures of the form $A^{HS} B^{ST} C^{TH}$.
%\begin{claim}
%	The amount of time it takes to create the data structures of the form $A^{HS} B^{ST} C^{TH}$  
%	for a vertex $v\in L_2$ transitioning from $T$ to $S$ is $m^{2/3+2\eps}$.
%\end{claim}
%\begin{proof}
%	We go over all $m^{1/3+\eps}$ neighbors of $v$ in $L_1^H$ and also all $m^{1/3+\eps}$ high 
%	degree vertices $w_i$ in $L_4$. 
%	We then use the number of paths between $v$ and $w_i$ through $L_3^T$ stored in 
%	$B^{AT}C^{TA}$ and create the data structure.	
%	This gives us the desired bound of $m^{2/3+2\eps}$ for the update time.
%\end{proof}
%
%
%Now consider vertices transitioning from $S$ to $T$.
%The amount of time we have is $m^{1/3-2\eps} \cdot m^{2/3-\eps}=m^{1-3\eps}$.
%
%We start with the data structure $A^{AT} B^{TA}$.
%\begin{claim}
%	The amount of time it takes to create the data structure $A^{AT} B^{TA}$ for a vertex 
%	$v$ transitioning from $S$ to $T$ is $O(m^{2/3-4\eps})$.
%\end{claim}
%\begin{proof}
%	We go over all pairs of $m^{1/3-2\eps}$ neighbors on both sides and create the data structure.
%\end{proof}
%
%Next consider the data structures of the form $A^{MT} B^{TT}C^{TH}$.
%\begin{claim}
%	The amount of time it takes to create the data structure $A^{MT} B^{TT}C^{TH}$ for a vertex 
%	$v\in L_2$ transitioning from $S$ to $T$ is $m^{2/3-\eps}$.
%\end{claim}
%\begin{proof}
%	We go over all $m^{1/3-2\eps}$ neighbors of $v$ in $L_1^M$ and also all $m^{1/3+\eps}$ high 
%	degree vertices $w_i$ in $L_4$. 
%	We then use the number of paths between $v$ and $w_i$ through $L_3^T$ stored in 
%	$B^{AT}C^{TA}$ and create the data structure.	
%	This gives us the desired bound of $m^{2/3-\eps}$ for the update time.
%\end{proof}
%
%Finally, consider the data structures of the form $A^{HT} B^{TS} C^{SH}$.
%\begin{claim}
%	The amount of time it takes to create the data structures of the form $A^{HT} B^{TS} C^{SH}$
%	for a vertex $v\in L_2$ transitioning from $S$ to $T$ is $m^{2/3-\eps}$.
%\end{claim}
%\begin{proof}
%	We go over all $m^{1/3-2\eps}$ neighbors of $v$ in $L_1^H$ and also all $m^{1/3+\eps}$ high 
%	degree vertices $w_i$ in $L_4$. 
%	We then use the number of paths between $v$ and $w_i$ through $L_3^S$ stored in 
%	$B^{AS}C^{SA}$ and create the data structure.	
%	This gives us the desired bound of $m^{2/3-\eps}$ for the update time.
%\end{proof}
%
%
%\vihan{also how to update the DS when phases change}
%
%
%
%\subsection{Constraints}
%We want to maximize $\eps$.
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%


==> figs/Join1.tex <==
\begin{tikzpicture}
	\node[vertexA] at (0,0) (a1) {};
	\node[vertexA] at (0,1) (a2) {};
	\node[vertexA] at (0,2) (a3) {};
	\node[vertexA] at (2,0) (b1) {};
	\node[vertexA] at (2,1) (b2) {};
	\node[vertexA] at (2,2) (b3) {};
	
	\node[vertexA] at (4,0) (c1) {};
	\node[vertexA] at (4,1) (c2) {};
	\node[vertexA] at (4,2) (c3) {};
	
	\node[vertexA] at (6,0) (d1) {};
	\node[vertexA] at (6,1) (d2) {};
	\node[vertexA] at (6,2) (d3) {};
	
		
	\draw[edge] (a1) -- (b3);
	\draw[edge] (a2) -- (b2);
	\draw[edge] (a1) -- (b1);
	\draw[edge] (a1) -- (b2);
	\draw[edge] (a3) -- (b2);
	
	\draw[edge] (c3) -- (d1);
	\draw[edge] (c3) -- (d3);
	\draw[edge] (c2) -- (d1);
	\draw[edge] (c1) -- (d1);
	
	% Text Node
	\draw (1,-0.5) node [anchor=north west][inner sep=0.75pt]   [align=left] 
	{\scriptsize{$A$}};
	
	% Text Node
	\draw (5,-0.5) node [anchor=north west][inner sep=0.75pt]   [align=left] 
	{\scriptsize{$B$}};

	% Text Node
\draw (0,3) node [anchor=north west][inner sep=0.75pt]   [align=left] 
{\scriptsize{$L_1$}};

	% Text Node
\draw (2,3) node [anchor=north west][inner sep=0.75pt]   [align=left] 
{\scriptsize{$L_2$}};

	% Text Node
\draw (4,3) node [anchor=north west][inner sep=0.75pt]   [align=left] 
{\scriptsize{$L_2$}};

	% Text Node
\draw (6,3) node [anchor=north west][inner sep=0.75pt]   [align=left] 
{\scriptsize{$L_3$}};


% Text Node
\draw (-0.7,2.2) node [anchor=north west][inner sep=0.75pt]   [align=left] 
{\scriptsize{$3$}};
	
% Text Node
\draw (-0.7,1.2) node [anchor=north west][inner sep=0.75pt]   [align=left] 
{\scriptsize{$2$}};

% Text Node
\draw (-0.7,0.2) node [anchor=north west][inner sep=0.75pt]   [align=left] 
{\scriptsize{$1$}};	
	
\end{tikzpicture}

==> figs/LayeredGraph.tex <==
\begin{tikzpicture}
	\node[vertexA] at (0,0) (a1) {};
	\node[vertexA] at (0,1) (a2) {};
	\node[vertexA] at (0,2) (a3) {};
	\node[vertexA] at (2,0) (b1) {};
	\node[vertexA] at (2,1) (b2) {};
	\node[vertexA] at (2,2) (b3) {};
	
	\node[vertexA] at (4,0) (c1) {};
	\node[vertexA] at (4,1) (c2) {};
	\node[vertexA] at (4,2) (c3) {};
	
	\node[vertexA] at (6,0) (d1) {};
	\node[vertexA] at (6,1) (d2) {};
	\node[vertexA] at (6,2) (d3) {};
	
	\node[vertexA] at (0,0) (u1) {};
	\node[vertexA] at (0,1) (u2) {};	
	\node[vertexA] at (0,2) (u3) {};
	
	\node[vertexA] at (0,0) (v1) {};
	\node[vertexA] at (2,1) (v2) {};
		
	\draw[edge] (a1) -- (b3);
%	\draw[edge] (a2) -- (b1);
%	\draw[edge] (a2) -- (b3);
%	\draw[edge] (a3) -- (b3);
	\draw[edge] (a2) -- (b2);
	\draw[edge] (a1) -- (b1);
	\draw[edge] (a1) -- (b2);
	\draw[edge] (a3) -- (b2);
	
	% Text Node
	\draw (1,-0.5) node [anchor=north west][inner sep=0.75pt]   [align=left] 
	{\scriptsize{$A$}};
	
% Text Node
\draw (3,-0.5) node [anchor=north west][inner sep=0.75pt]   [align=left] 
{\scriptsize{$B$}};

% Text Node
\draw (5,-0.5) node [anchor=north west][inner sep=0.75pt]   [align=left] 
{\scriptsize{$C$}};
	
%Shape: Rectangle [id:dp7888938918159529] 
\draw   (1.7,2.2) -- (2.3,2.2) -- (2.3,1.3) -- (1.7,1.3) -- cycle ;

% Text Node
\draw (1.9,2.5) node [anchor=north west][inner sep=0.75pt]   [align=left] 
{\scriptsize{$D$}};


	
\end{tikzpicture}

==> layered_paws.tex <==
% !TeX root = main.tex 
%!TEX root = main.tex

\section{Extending the Algorithm to \texorpdfstring{$4$}{4}-Paws in Layered Graphs}

\vihan{is there a faster alg for tri counting?}

In this section, we present an algorithm to count $4$-paws in layered graphs in time 
$O(m^{2/3-\eps})$.


\subsection{Counting the Number of Triangles through a Vertex}

Say we are given a $3$-layer graph $G$, and we want to maintain the number of triangles that go 
through a vertex.
We can easily solve this problem by using our algorithm for counting the number of $3$-paths 
between pairs of vertices.

Construct a $4$-layer graph $G'$ from the $3$-layer graph $G$ by repeating the first layer as the 
fourth layer and add the edges between $L_3$ and $L_4$ instead of $L_3$ and $L_1$.
Now computing the number of triangles through a vertex $v$ in the original graph $G$ can be done 
by finding the number of paths from $v$ to $v$ in $G'$.
Our algorithm solves this problem in time $O(m^{2/3-\eps})$ so we get an algorithm for counting the 
number of triangles though a vertex in worst-case update time $O(m^{2/3-\eps})$.



\subsection{Setup for Paws}

We maintain two separate algorithms for edge insertions between different layers.
If the edge update is incident on $L_2$ then the algorithm to solve the problem is simple.
If the edge $(u,v)$ is between $L_2$ and $L_3$ then we query the number of triangles through $u$ 
and output that as the number of new paws using $(u,v)$.
Otherwise, if the edge $(u,v)$ is between $L_1$ and $L_2$ then we query the number of $2$-paths 
between $u$ and $v$ through $L_4$ and multiply that by the degree of $v$ to $L_3$.
The algorithm is symmetric for edge update between $L_2$ and $L_4$.
Note that all these computations can be done in time $O(m^{2/3-\eps})$.

Thus, the hard case is when the edge update is between $L_1$ and $L_4$.
We now focus on answering queries only in this case.
Let the query edge $(u,v)$ be between $L_1$ and $L_4$.
Let $A$ be the matrix of edges between $L_1$ and $L_2$ and $C$ is the matrix of edges between 
$L_2$ and $L_4$. Finally, $B$ is the matrix of edges between $L_2$ and $L_3$.
The edge updates to $B$ are divided into \textbf{chunks} of size $m^{2/3 - \eps}$ called 
$B_1,B_2,\ldots B_i$ (similar to \Cref{sec:setup-simple}).


We now state the assumptions we need in this section:
\begin{restatable}{assumption}{AsmPawConstAC}\label{asm:paw-AC-constant}
	There are no edge updates in $A$ and $C$ i.e.\ the only edge updates are in $B,D$.
\end{restatable}

\begin{restatable}{assumption}{AsmPawMatching}\label{asm:paw-matching}
	The edges in each chunk $B_i$ form a matching.
\end{restatable}


\subsection{Data Structures}

Here we mention the data structures we need to store.
We need to store the number of stars $x,y$ are a part of where $x \in L_1$ and $y\in L_4$.
If we fix a chunk $B_i$ for this data structure then we are counting the number of $2$-paths from 
$x$ to $y$ through $L_2$.

\begin{claim}\label{clm:stars-low-deg-verts-pawAlg}
	Given $x\in L_1$ and $y \in L_4$ where $\deg(x) \leq m^{2/3-\eps}$ or $\deg(y) \leq 
	m^{2/3-\eps}$, computing the number of stars between $x$ and $y$ can be done in time 
	$O(m^{2/3-\eps})$.
\end{claim}
\begin{proof}
	In this case, when we get a query for the number of stars including $x,y$ we can iterate over their 
	common neighbors in time $m^{2/3-\eps}$. For each of those vertices we sum up their degree to 
	$L_3$ to get the answer to the query.	
\end{proof}

Now we can focus on the case where $\deg(x) \geq m^{2/3-\eps}$ and $\deg(y) \geq 
m^{2/3-\eps}$.
There are $m^{1/3+\eps}$ such \textbf{high degree} vertices in $L_1$ and $L_4$.
Let $B$ be the set of vertices in $L_2$ $B_i$ is incident on.
Let $A^{HB}$ be the submatrix of $A$ incident on the high degree vertices in $L_1$ and $B$ in 
$L_2$.
Similarly, let $C^{BH}$ be the submatrix of $C$ incident on $B$ in $L_2$ and the high degree 
vertices in $L_4$.
We can multiply $A^{HB}$ and $C^{BH}$ in time $m^{\omega(1/3+\eps,2/3-\eps,1/3+\eps)}$.
We need this to be at most $m^{4/3-2\eps}$ so we get the constraint:
\begin{constraint}\label{eq:DS-AC-paw}		
	\omega(1/3+\eps,2/3-\eps,1/3+\eps)\leq 4/3 -2\eps.
\end{constraint}



\subsection{Queries}

Let the current query be $e=(u,v)$ where $u$ is in $L_1$ and $v$ is in $L_4$.
Let $B_{i+1}$ be the current chunk in $B$ that was being inserted when we got query $e$.  
Note that the chunk $B_{i+1}$ might be incomplete.

We use the procedure of \emph{lazy evaluation} from \Cref{subsec:queries-simple} for chunks 
$B_i$ and $B_{i+1}$.
Given the query $u,v$ we go over all edges of $B_i$ one by one and check if it forms a star with 
$u$ and $v$ (similar for $B_{i+1}$). This takes $O(1)$ time per edge in $B_i$. Thus, we know the 
number of stars with $u$ and $v$ using edges of $B_i$ and $B_{i+1}$.
We now have to only look at paths that go through $B_{<i} := \cup_{j=1}^{i-1} B_j$.


We know using \Cref{clm:stars-low-deg-verts-pawAlg} that if the query $(u,v)$ has $\deg(u) \leq 
m^{2/3-\eps}$ or $\deg(v) \leq 
m^{2/3-\eps}$, computing the number of stars between $u$ and $v$ can be done in time 
$O(m^{2/3-\eps})$.
During the insertion of chunk $B_i$, we compute $A^{HB} \cdot C^{BH}$ in time 
$m^{\omega(1/3+\eps,2/3-\eps,1/3+\eps)} \leq m^{4/3-2\eps}$ (\Cref{eq:DS-AC-paw}).
Thus, we have the number of stars between $u$ and $v$ stored when both $u$ and $v$ have a high 
degree.
Therefore, we can answer the query in time $O(m^{2/3-\eps})$. 


\subsection{Removing Assumptions}

It is very easy to get rid of \Cref{asm:paw-matching}.
We need to show how to modify the data structure $A^{HB} \cdot C^{BH}$ for the number of stars 
because now we need to count weighted paths instead of paths.
If $B_i$ is not a matching then we can create a new vertex for each edge in $B_i$ and call this layer 
$B'$. The neighborhood in $L_1$ and $L_4$ of a vertex $(x,y)$ in $B'$ is the same as the 
neighborhood of $x$. 
Let $A^{HB'}$ be the matrix of edges between $L_1^H$ and $B'$.
Compute $C^{B' H}$ similarly and multiply them instead of $A^{HB} \cdot C^{BH}$.
The complexity remains the same because the number of vertices in $B'$ is $m^{2/3-\eps}$.

We now discuss how to get rid of \Cref{asm:paw-AC-constant}.

Say that there are edge updates in $A$ and $C$.
We need to update the stored data structure $A^{HB'} \cdot C^{B' H}$.
Consider the edge update $(u,v)$ in $A$ (the analysis for $C$ is symmetric).
We need to update the data structure only if $u \in L_1^H$ so let's assume that is the case.
We then iterate over all the vertices $w$ in $L_4^H$.
If $w$ is a neighbor of $v$ then we update the number of stars between $u$ and $w$ by degree of 
$v$ to $L_3$.
This takes time $m^{1/3+\eps} \leq m^{2/3-\eps}$. 



==> prelim-old.tex <==
% !TeX root = main.tex 
%!TEX root = main.tex


\section{Preliminaries}\label{sec:prelim}

\paragraph{Notation.}
For a graph $G=(V,E)$, we use $n$ to represent the number of vertices and $m$ to represent the 
number of edges.
We use $\deg(v)$ and $N(v)$ for each vertex $v \in V$ to denote the degree 
and neighborhood of $v$, respectively. For a subset $F$ of edges in $E$, we use $V(F)$ to denote 
the vertices incident on $F$; similarly, for a set $U$ of vertices, $E(U)$ denotes the edges 
incident on $U$. We further use $G[U]$ for any set $U$ of vertices to denote the induced subgraph 
of $G$ on $U$. 

We now discuss some notation for fast matrix multiplication.
Note that $\omega$ is the exponent of square matrix multiplication. 
This means that the time it takes 
to multiply two $n \times n$ matrices is $O(n^{\omega})$.
The current best known upper bound on $\omega$ is $2.371339$ 
\cite{alman2024more}.
We will also need fast rectangular matrix multiplication in our algorithm.
We define $\omega(a,b,c)$ to be the exponent of rectangular matrix multiplication 
of an $n^a \times 
n^b$ dimension matrix by an $n^b \times n^c$ dimension matrix.
\cite{alman2024more} also gives improved upper bounds for $\omega(a,b,c)$.

Let the layers of the $4$-layered graph be $L_1,L_2,L_3, L_4$.
Throughout the paper, we are solely focused on layered graphs with $4$ number of 
layers.
%Any $4$-vertex subgraph whose copies we are trying to count in a $4$-layered 
%graph has to have 
%exactly one vertex in each of the $4$ layers and appropriate edges between 
%those vertices.
A layered $4$-cycle in a layered graph has exactly one vertex in each layer and edges 
connecting a vertex in a layer to the vertex in the next layer.
The cycle cannot have one vertex in $L_1$ and $L_3$ each and two vertices in 
$L_2$ even though that is a valid cycle in a general graph.
For convenience, we will drop the word ``layered'' and call a layered $4$-cycle a $4$-cycle, because we will 
only deal with layered $4$-cycle in $4$-layered graphs.
Similarly, a $3$-path in a $4$-layer graph is a path containing $4$ vertices, where each vertex is in a 
distinct layer, and they have edges between them (so a $4$-cycle in a $4$-layered 
graph minus an edge). 

%Note that it is not enough for all vertices to be distinct, the also have to be in 
%distinct layers.


%We now formally define all the different types of $4$ vertex subgraphs in 
%$4$-layered graphs.
%The other types of $4$ vertex subgraphs are the same as these up to 
%permutations of vertices.
%Let the $4$ vertices in $L_1,L_2,L_3,L_4$ be $v_1,v_2,v_3,v_4$ respectively. 
%We then have the following 
%types of $4$ vertex subgraphs:
%\begin{itemize}
%	\item $3$-path: An edge between $(v_1,v_2)$, $(v_2,v_3)$ and $(v_3,v_4)$.
%	\item $4$-cycle: An edge between $(v_1,v_2)$, $(v_2,v_3)$, $(v_3,v_4)$ and 
%$(v_4,v_1)$.
%	\item $4$-star: An edge between $(v_1,v_2)$, $(v_1,v_3)$, and $(v_1,v_4)$.
%	\item $4$-paw: An edge between $(v_1,v_2)$, $(v_2,v_3)$, $(v_2,v_4)$ and 
%$(v_1,v_4)$.	
%	\item $4$-diamond: An edge between $(v_1,v_2)$, $(v_2,v_3)$, 
%$(v_3,v_4),(v_4,v_1)$ and 
%	$(v_1,v_3)$.
%	\item $4$-clique: An edge between $(v_1,v_2)$, $(v_2,v_3)$, 
%$(v_3,v_4),(v_1,v_3)(v_1,v_4)$ 
%	and $(v_2,v_4)$.
%\end{itemize}


%\vihan{should we call the layers $0,1,2,3$ bec then mod works? We might want to 
%say layer i and i+1 to be 
%4 and 1}

\begin{comment}
\paragraph{Equivalent Problems.}
The problem we are interested in is maintaining the total number of $4$-cycles in a general graph in the 
fully dynamic model.
It is easy to observe that this problem is equivalent to just counting the number of new cycles that go 
through the latest edge update.
Let the latest edge update be $(u,v)$.
Counting the number of new cycles that go through $(u,v)$ is equivalent to counting the number of 
$3$-paths from $u$ to $v$.
Surprisingly enough, counting the number of $3$-paths from $u$ to $v$ is equivalent to counting the 
number of $3$-walks from $u$ to $v$.
\begin{claim}
	In a simple graph where $(u,v) \not\in E$, the number of walks of length $3$ from $u$ to $v$ is equal 
	to the number of 
	paths of length $3$ from $u$ to $v$.
\end{claim}
\begin{proof}
	Consider a walk $u,x,y,v$ of length $3$ from $u$ to $v$.
	We will show that this is a path which means that all vertices are distinct.
	
	Firstly we have $x \neq u$ because we do not have self loops (edges of the form $(i,i)$).
	Also, $x \neq v$ because the edge $(u,v)$ does not exist.
	The same arguments show that $y \neq u$ and $y \neq v$.
	Finally, we have $x \neq y$ because we do not have self loops.
	Thus, all the vertices are distinct and $u,x,y,v$ is a path.
\end{proof}

By a similar reasoning, maintaining the total number of $4$-cycles in a layered graph is equivalent to  
counting the number of new cycles that go through the latest edge update which is equivalent to just 
counting the number of $3$-paths between pairs of vertices.

Finally, if we have an algorithm to count the number of $3$-paths in layered graphs, we can come up with 
an algorithm to count $3$-walks in general graphs in the following way.
We add all vertices $V$ of the general graph to all the $4$ layers and then use the algorithm to count the 
number of $3$-paths in layered graphs and count the number of 
$3$-paths between the first and the last layer.
This gives us the number of $3$-walks in the general graph because all the layers contain all the vertices.


The other direction is trivial because layered graphs are a subset of general graphs so any algorithm for 
general graphs directly works for layered graphs. 
This shows that maintaining the number of $4$-cycles in general graphs is equivalent to maintaining the 
number of $4$-cycles in layered graphs.
The equivalent version of the problem we will solve in this paper is counting the number of $3$-paths in 
layered graphs.
\end{comment}

\paragraph{Setup for Cycle Counting in Layered Graphs.}
We have four layers $L_1,L_2,L_3$ and $L_4$ each containing $n$ vertices.
Let the edges between the four consecutive layers be represented by the matrices 
$A, B, 
C,$ and $D$. 
It is easy to see that maintaining the total number of $4$-cycles is equivalent to just counting the 
number of new cycles i.e.\ cycles that go through the new edge update.
We answer the query of the number of new cycles by counting the number of $3$-paths between 
the endpoints of the edge update.
%We have already shown that counting the total number of $4$-cycles in a layered graph is 
%equivalent to 
%counting the number of $3$-paths between arbitrary pairs of vertices.
We assume without loss of generality that we have to answer queries only when there is an edge 
update in $D$ because we run $4$ copies of this algorithm, one for queries in $D$ and the others 
for queries in $A,B,$ and $C$.
This means that queries are in $D$ but edge updates are in $A,B,$ and $C$, so we 
maintain data structures that help us answer queries in $D$. 
Note that we maintain the same data structures for all $4$ copies of the algorithm 
(corresponding to matrices $A,B,C$ and $D$). By symmetry, the analysis is the 
same for all of them, so we just focus on the case when queries are in $D$ and 
edge updates are everywhere else.






